The Zero Turbulence Manifold in Fusion Plasmas

The transport of heat that results from turbulence is a major factor limiting the temperature gradient, and thus the performance, of fusion devices. We use nonlinear simulations to show that a toroidal equilibrium scale sheared flow can completely suppress the turbulence across a wide range of flow gradient and temperature gradient values. We demonstrate the existence of a bifurcation across this range whereby the plasma may transition from a low flow gradient and temperature gradient state to a higher flow gradient and temperature gra- dient state. We show further that the maximum temperature gradient that can be reached by such a transition is limited by the existence, at high flow gradient, of subcritical turbulence driven by the parallel velocity gradient (PVG). We use linear simulations and analytic calculations to examine the properties of the transiently growing modes which give rise to this subcritical turbulence, and conclude that there may be a critical value of the ratio of the PVG to the suppressing perpendicular gradient of the velocity (in a tokamak this ratio is equal to q/{\epsilon} where q is the magnetic safety factor and {\epsilon} the inverse aspect ratio) below which the PVG is unable to drive subcritical turbulence. In light of this, we use nonlinear simulations to calculate, as a function of three parameters (the perpendicular flow shear, q/{\epsilon} and the temperature gradient), the surface within that parameter space which divides the regions where turbulence can and cannot be sustained: the zero- turbulence manifold. We are unable to conclude that there is in fact a critical value of q/{\epsilon} below which PVG-driven turbulence is eliminated. Nevertheless, we demonstrate that at low values of q/{\epsilon}, the maximum critical temperature gradient that can be reached without generating turbulence is dramatically increased.

==> thesis-partv.tex <==
%
\mypart{Conclusions}
\label{conclusions}
We have determined the way the turbulent transport of heat
and toroidal angular momentum
is affected by the equilibrium gradients of temperature and velocity
over a wide range of those two parameters,
in the case of a plasma with a sonic background flow\footnote{
We have neglected the effect of the Coriolis force due to such a flow in our study. 
However, previous work \cite{peeters2007toroidal} indicates that its effect is to reduce the effective turbulent momentum diffusivity through a momentum pinch. 
This will make higher-flow-shear regimes easier to access but will not affect the bifurcation mechanism,
since the neoclassical transport of momentum remains much lower.
}.
We have extended the range of flow shears up to 20 times
the linear ITG instability growth rate 
calculated at zero flow shear. 
We have considered the zero-magnetic-shear regime.
We have used a low value of the safety factor, $q_0=1.4$,
which reduces the strength of the destabilising parallel velocity gradient drive
relative to the stabilising perpendicular velocity shear.
In so doing we have established the following key results:

\begin{enumerate}
	\item 
		The plasma is linearly stable to microinstabilities for all non-zero values of flow shear but subcritical turbulence can be sustained nonlinearly across much of this stable region.
	\item
		For velocity shear \(\fsr\lesssim 1\) 
		(we remind our readers that $\fsr$ is normalised to $v_{thi}/R_0$),
		increasing $\fsr$ 
		reduces the levels of turbulence
		driven by the ion temperature gradient.
		For \(\fsr\gtrsim 1\),
		the destabilising effect of the parallel velocity gradient
		becomes dominant and 
		increasing the flow shear increases the levels of turbulence and turbulent transport.
	\item
		For low flow shears, $\fsr\leq0.8$,
		and low heat flux, \(Q_t/Q_{gB}\lesssim2.5 \),
		flow shear reduces the thermal transport stiffness. 
		For low flow shears and higher $Q_t$, flow shear increases the thermal transport stiffness. 
		At high flow shears, $\fsr\gtrsim1$, the thermal stiffness is reduced as the PVG drive becomes dominant. 
	\item 
		For $\fsr\gtrsim0.1$
		the turbulent Prandtl number stays within the range 0.5--0.8
		across a wide range of temperature gradients.
		Thus, the turbulence transports heat and momentum with comparable vigour.

	\item
		For \(R_0/L_T\lesssim 11\),
		there is a large region around \(\fsr\sim1\)
		where the turbulence is completely quenched.
	\item
		Owing to the existence of this region,
		and the fact that the neoclassical Prandtl number
		is much lower than the turbulent Prandtl number,
		it is possible to trigger a bifurcation
		to a regime of high velocity and temperature gradients
		by either (i) increasing the momentum input at constant heat input
		or (ii) lowering \(Q/Q_{gB}\) at a constant ratio of heat to momentum input.
	\item
		In the high gradient (reduced transport) state
		that is reached via this bifurcation,
		the heat is principally transported neoclassically,
		whereas the momentum is principally transported by turbulence.
	\item
		For any given input of toroidal angular momentum, 
		there is an optimum input of of heat which maximises the temperature gradient. 
		Increasing the input of heat above this optimum
		can reduce the temperature gradient
		by increasing the levels of turbulence.
\end{enumerate}







	







